SPARSER: Sparse Variable Projection by Exploiting Separable Structure in Robotic Perception

Robotic perception often requires solving large nonlinear least-squares (NLS) problems. While sparsity has been well exploited to scale solvers, separability remains underexploited: some variables (e.g., landmarks) appear linearly in the residuals and admit a closed-form solution once the others (e.g., poses) are fixed. Variable projection (VarPro) exploits this by analytically eliminating the linear variables, yielding a reduced problem with favorable properties. However, VarPro is rarely used in robotic perception, largely because gauge symmetries (e.g., invariance to global shifts and rotations), common in perception, complicate standard VarPro approaches. We present SPARSER (Sparsity Preserving Analytic Reduction for Separable Estimation in Robotics), a VarPro scheme for problems with gauge symmetries that jointly exploits separability and sparsity. Via one-time preprocessing, it builds a matrix-free Schur complement operator that evaluates costs, gradients, and Hessian-vector products of the reduced problem and integrates with standard iterative NLS solvers. We characterize the applicable problem class and common special cases admitting further analytical savings. The method extends to robust costs via iteratively reweighted least squares (IRLS): symbolic preprocessing is reused across reweightings, so each IRLS iteration needs only a numerical refactorization. On 42 benchmark datasets spanning pose-graph optimization, range-aided SLAM, sensor network localization, and structure from motion, SPARSER is fastest on 41 on CPU and 35 on GPU, and is the only method to solve all. On 24 real-world multi-robot SLAM datasets with outlier-corrupted loop closures, our robust variant is the only method to solve all and is fastest on each, running 1.1-3.1x faster than the graduated non-convexity (GNC) solver in GTSAM. We release open-source C++ code and all datasets.

==> tab/cora_vs_dcora_absolute_trajectory_error.tex <==
\begin{table}[!t]
\renewcommand{\arraystretch}{1.0}
\caption{DCORA vs. CORA on Public Real-World Multi-Agent RA-SLAM Datasets}
\label{tab:cora_vs_dcora_absolute_trajectory_error}

\begin{threeparttable}
    \setlength{\tabcolsep}{5.5pt}
    
    %% Table
    \begin{tabularx}{\columnwidth}{cc cc cc}
    \toprule
    \multirow{2}{*}{\textbf{Dataset\tnote{$\dagger$}}} & 
    \multirow{2}{*}{\textbf{Algorithm}} & 
    \multicolumn{2}{c}{\textbf{Certification\tnote{$\ddagger$}}} &
    \multicolumn{2}{c}{\textbf{ATE (RMSE)\tnote{$\ast$}}} \\
    & 
    & \textbf{$f^{\ast}_{\text{SDP}}$}
    & \textbf{$\epsilon$}
    & \textbf{Trans. [m]}
    & \textbf{Rot. [\degree{}]} \\
    \midrule    
    \multirow{2}{*}{\texttt{TIERS} }
    & DCORA & 1920.4 & 1e-2 & 0.04 & 0.05 \\
    & CORA  & 1921.9 & 1e-3 & 0.04 & 0.05 \\
    \midrule
    \multirow{2}{*}{\texttt{MR.CLAM 2} } 
    & DCORA & 7032.9 & 5e-3 & \textbf{0.15} & 0.12 \\
    & CORA  & 7034.6 & 1e-3 & 0.17 & 0.12 \\
    \midrule
    \multirow{2}{*}{\texttt{MR.CLAM 4} }
    & DCORA & 4173.2 & 5e-3 & 0.13 & 0.10 \\
    & CORA  & 4173.1 & 1e-3 & 0.13 & 0.10 \\
    \midrule
    \multirow{2}{*}{\texttt{MR.CLAM 6} }
    & DCORA & 3124.8 & 5e-3 & 0.27 & 0.14 \\
    & CORA  & 3124.5 & 1e-3 & \textbf{0.26} & 0.14 \\
    \midrule
    \multirow{2}{*}{\texttt{MR.CLAM 7} }
    & DCORA & 3091.4 & 5e-2 & 0.31 & 0.14 \\
    & CORA  & 3038.4 & 1e-2 & \textbf{0.27} & \textbf{0.13} \\
    \bottomrule
    \end{tabularx}

    %% Footnotes
    \smallskip
    \scriptsize
    \begin{tablenotes}
    \RaggedRight
    \item[$\dagger$] Datasets include \texttt{TIERS}\cite{yu2023fusing} and sessions \texttt{2}, \texttt{4}, \texttt{6}, and \texttt{7} of \texttt{MR.CLAM}\cite{leung2011utias}.
    \item[$\ddagger$] All solutions are certified.
    \item[$\ast$] Bold values indicate best performance.
    \end{tablenotes}
    \end{threeparttable}
\vspace{-20pt}
\end{table}

%% \texttt{TIERS}

% ape_rot_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.04788667500270187,0.0374184851069051,0.035102260701938795,0.023850332685173246,0.004659969853255119,0.34671054844397853,7.308762040727498
% dcora,0.04851865292093692,0.03806860970964114,0.035938996472964,0.024225094845841635,0.0029248045199599176,0.34493049024365124,7.019599944593068

% ape_trans_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.03768974100956831,0.03369054696817231,0.03166070349323302,0.016832034148763476,0.0008761966088990838,0.0930442777795755,3.556735498927725
% dcora,0.04293710920738049,0.03898473475210604,0.0384801268040132,0.017956700100442473,0.0008258317723597541,0.09695497897342181,4.598448365105399

%% MRCLAM 2

% ape_rot_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.11880267098215903,0.07282495801589982,0.05247297249491891,0.09356446799221407,1.764866510923627e-05,2.6071152885741777,92.73780548635276
% dcora,0.1175462171274559,0.07207251373806359,0.05200583148745635,0.09253858096289577,1.3521548108266356e-05,2.606426027177529,90.9547533241587

% ape_trans_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.17029503320784306,0.13089158186153094,0.11214511088358045,0.10424274627666874,0.002320050530306387,1.1781610309684294,190.93802408359474
% dcora,0.15477272593259672,0.12833603347480954,0.11102317210174535,0.08585294113362159,0.0024355936036593914,0.698359059848473,151.12547049444842

%% MRCLAM 4

% ape_rot_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.10394471961737659,0.06497103626316045,0.04598912282725178,0.08097767106018822,8.872094366368605e-06,2.6614628633668795,58.78650724296125
% dcora,0.10386899117350122,0.06487609897467776,0.045844030787411644,0.08096604280455665,8.58436448201835e-06,2.6615400163490173,58.70330304271791

% ape_trans_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.13243819735070148,0.11577265076697861,0.10497073290856151,0.06423315874965235,0.0024244029489987355,0.45691423892003186,94.45307195514494
% dcora,0.13141364781797077,0.11518477871790919,0.10459417665874338,0.06316240453240783,0.0017168603334075847,0.4201296543467081,92.90528017283185

%% MRCLAM 6

% ape_rot_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.13792177044335494,0.09920851751553553,0.08156891037056462,0.09558359442066958,7.646289737166913e-05,2.107626478537017,44.36930186097884
% dcora,0.14087118851233488,0.10155796454201024,0.08592396941342434,0.09718718154455241,5.8338943389705055e-05,2.110025194535469,45.972339228504175

% ape_trans_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.2586082981855127,0.21567735447693148,0.18359074055251456,0.1411996158718999,0.004396138376510067,0.904936617455909,156.9804262735807
% dcora,0.272353032248827,0.2306788148738863,0.19733212148957957,0.14378890510427714,0.009899593151416232,0.8674212789741396,172.46862821236513

%% MRCLAM 7

% ape_rot_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.13303907442593757,0.08793838542289406,0.06476904524243719,0.09931819828502744,4.8841731671355083e-05,1.85881015846872,49.91607453352784

% ape_trans_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.27259569786413135,0.20524365202816355,0.1691962749802089,0.17440528402169947,0.006462333940518948,1.7672926591380969,222.0213520960355

%% Updated MRCLAM 7 tests. MRCLAM 7 experiments have been re-run with adjustments made to parameters to suit the conditions of the dataset. Note that we had to lower the gradient tolerance and preconditioned gradient tolerance to 1e-2 vs. 1e-4 as in the original CORA implementation.

% CORA (reimp): 
% min_eig_tol = 1e-3
% gradient_tolerance = 1e-2;
% preconditioned_gradient_tolerance = 1e-2;

% I0218 10:53:02.609759 29667 SingleRobotExample_RASLAM.cpp:199] Objective value at rank 15: 3045.13
% I0218 10:53:02.614893 29667 SingleRobotExample_RASLAM.cpp:201] Gradient norm at rank 15: 89.5362
% I0218 10:53:06.241750 29667 SingleRobotExample_RASLAM.cpp:221] Z = (X*)^T(X*) is a global minimizer!
% I0218 10:53:06.605778 29667 Graph.cpp:1956] Largest eigenvalue 157737 of P computed successfully for agent 0. Setting preconditioner regularization term to: 0.157737
% I0218 10:53:12.902541 29667 SingleRobotExample_RASLAM.cpp:237] Outputting rounded centralized trajectory for each agent.

% DCORA: 
% min_eig_tol = 5e-2
% gradient_tolerance = 1e-2;
% preconditioned_gradient_tolerance = 1e-2;

% I0218 16:14:14.089098 356313 MultiRobotExample_RASLAM.cpp:384] 2999 2  3091.421596 10.303316
% I0218 16:14:19.796433 356313 MultiRobotExample_RASLAM.cpp:485] Z = (X*)^T(X*) is a global minimizer! Outputting rounded agent trajectories.

% ape_rot_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% cora,0.13600249568612147,0.08824693415367066,0.06455923855908684,0.10281129268080591,3.637469981460872e-05,1.8742232247378432,52.3397265420132
% dcora,0.13787856426672274,0.0985108237803652,0.07599446046684866,0.09620918999710501,4.008897871430937e-05,1.8590511021110026,53.98531893121684

% ape_trans_stats.csv
% alg,rmse,mean,median,std,min,max,sse
% 
% alg,rmse,mean,median,std,min,max,sse
% cora,0.276144804399181,0.20585845186127727,0.16898457894120952,0.17872018971886558,0.006758242143058131,1.8177150427169062,228.60122945180842
% dcora,0.30615554249321275,0.23820103471057286,0.1808469510515354,0.18988964560003715,0.01439663753954076,1.224581744859492,271.56509874559816

